Computational modeling of the nonlinear stochastic dynamics of horizontal drillstrings

This work intends to analyze the nonlinear stochastic dynamics of drillstrings in horizontal configuration. For this purpose, it considers a beam theory, with effects of rotatory inertia and shear deformation, which is capable of reproducing the large displacements that the beam undergoes. The friction and shock effects, due to beam/borehole wall transversal impacts, as well as the force and torque induced by bit-rock interaction, are also considered in the model. Uncertainties of bit-rock interaction model are taken into account using a parametric probabilistic approach. Numerical simulations have shown that the mechanical system of interest has a very rich nonlinear stochastic dynamics, which generate phenomena such as bit-bounce, stick-slip, and transverse impacts. A study aiming to maximize the drilling process efficiency, varying drillstring velocities of translation and rotation is presented. Also, the work presents the definition and solution of two optimizations problems, one deterministic and one robust, where the objective is to maximize drillstring rate of penetration into the soil respecting its structural limits.

==> old.tex <==
%In this section, the modal content of the mechanical system
%is investigated. This investigatation aims to identify the natural 
%frequencies of the system, observe the shape of the normal modes
%(which are used in the construction the reduced model), and, especially,
%to check the influence of the fluid mass in the normal modes form.
%
%
%Several natural frequencies of the system can be seen in 
%Table~\ref{natural_freq_tab}, as well as the corresponding mechanism 
%of vibrations (rigid body, flexural, torsional or longitudinal). The six 
%rigid body modes that appear in the table reflect the fact that
%the geometric boundary conditions are imposed as constraints.
%Remember that the weak formulation refers to a free-free beam. 
%When the constraints are taken into account, the beam has only 
%two rigid body modes. Specifically, one longitudinal, and another torsional.
%It may also be noted that the lowest natural frequencies are associated 
%with the flexural mechanism. This is because the flexural stiffness of the 
%beam is much smaller than the torsional stiffness, which in turn is less 
%than the axial stiffness. In other words, it is much easier to bend the beam 
%than twisting it. However, twists the beam is easier than buckling it.
%
%
%\begin{table}[h!]
%	\centering
%	\caption{Normal modes used in the construction of the reduced model for
%	the mechanical system ($300~m$ long beam), and the corresponding natural frequencies.}
%	\begin{tabular}{ccl|ccl}
%		\toprule
%		mode & frequency (Hz) & type & mode & frequency (Hz) & type\\
%		\midrule
%    1 &     0.00 & rigid boby    &    70 &     4.12 & flexural in y\\
%    2 &     0.00 & rigid boby    &    71 &     4.12 & flexural in z\\
%    3 &     0.00 & rigid boby    &    72 &     4.37 & flexural in z\\
%    4 &     0.00 & rigid boby    &    73 &     4.37 & flexural in y\\
%    5 &     0.00 & rigid boby    &    74 &     4.64 & flexural in z\\
%    6 &     0.00 & rigid boby    &    75 &     4.64 & flexural in y\\
%    7 &     0.01 & flexural in y &    76 &     4.91 & flexural in z\\
%    8 &     0.01 & flexural in z &    77 &     4.91 & flexural in y\\
%    9 &     0.02 & flexural in z &    78 &     5.19 & flexural in z\\
%   10 &     0.02 & flexural in y &    79 &     5.19 & flexural in y\\
%   11 &     0.05 & flexural in y &    80 &     5.48 & flexural in y\\
%   12 &     0.05 & flexural in z &    81 &     5.48 & flexural in z\\
%   13 &     0.08 & flexural in y &    82 &     5.78 & flexural in y\\
%   14 &     0.08 & flexural in z &    83 &     5.78 & flexural in z\\
%   15 &     0.12 & flexural in y &    84 &     6.08 & flexural in z\\
%   16 &     0.12 & flexural in z &    85 &     6.08 & flexural in y\\
%   17 &     0.16 & flexural in y &    86 &     6.39 & flexural in y\\
%   18 &     0.16 & flexural in z &    87 &     6.39 & flexural in z\\
%   19 &     0.22 & flexural in y &    88 &     6.71 & flexural in y\\
%   20 &     0.22 & flexural in z &    89 &     6.71 & flexural in z\\
%   21 &     0.28 & flexural in y &    90 &     6.86 & torsional    \\
%   22 &     0.28 & flexural in z &    91 &     7.04 & flexural in y\\
%   23 &     0.35 & flexural in y &    92 &     7.04 & flexural in z\\
%   24 &     0.35 & flexural in z &    93 &     7.37 & flexural in z\\
%   25 &     0.43 & flexural in y &    94 &     7.37 & flexural in y\\
%   26 &     0.43 & flexural in z &    95 &     7.72 & flexural in y\\
%   27 &     0.52 & flexural in z &    96 &     7.72 & flexural in z\\
%   28 &     0.52 & flexural in y &    97 &     8.07 & flexural in y\\
%   29 &     0.61 & flexural in z &    98 &     8.07 & flexural in z\\
%   30 &     0.61 & flexural in y &    99 &     8.43 & flexural in y\\
%   31 &     0.71 & flexural in y &   100 &     8.43 & flexural in z\\
%   32 &     0.71 & flexural in z &   101 &     8.45 & longitudinal \\
%   33 &     0.82 & flexural in z &   102 &     8.79 & flexural in y\\
%   34 &     0.82 & flexural in y &   103 &     8.79 & flexural in z\\
%   35 &     0.94 & flexural in z &   104 &     9.17 & flexural in y\\
%   36 &     0.94 & flexural in y &   105 &     9.17 & flexural in z\\
%   37 &     1.06 & flexural in z &   106 &     9.55 & flexural in z\\
%   38 &     1.06 & flexural in y &   107 &     9.55 & flexural in y\\
%   39 &     1.19 & flexural in z &   108 &     9.94 & flexural in y\\
%   40 &     1.19 & flexural in y &   109 &     9.94 & flexural in z\\
%   41 &     1.33 & flexural in y &   110 &    10.29 & torsional    \\
%   42 &     1.33 & flexural in z &   111 &    10.34 & flexural in y\\
%   43 &     1.48 & flexural in y &   112 &    10.34 & flexural in z\\
%   44 &     1.48 & flexural in z &   113 &    10.74 & flexural in z\\
%   45 &     1.64 & flexural in z &   114 &    10.74 & flexural in y\\
%   46 &     1.64 & flexural in y &   127 &    13.72 & torsional    \\
%   47 &     1.80 & flexural in y &   142 &    16.90 & longitudinal \\
%   48 &     1.80 & flexural in z &   143 &    17.15 & torsional    \\
%   49 &     1.97 & flexural in y &   158 &    20.58 & torsional    \\
%   50 &     1.97 & flexural in z &   171 &    24.01 & torsional    \\
%   51 &     2.15 & flexural in z &   176 &    25.35 & longitudinal \\
%   52 &     2.15 & flexural in y &   183 &    27.44 & torsional    \\
%   53 &     2.34 & flexural in y &   194 &    30.87 & torsional    \\
%   54 &     2.34 & flexural in z &   203 &    33.79 & longitudinal \\
%   55 &     2.53 & flexural in y &   206 &    34.30 & torsional    \\
%   56 &     2.53 & flexural in z &   215 &    37.73 & torsional    \\
%   57 &     2.74 & flexural in y &   226 &    41.16 & torsional    \\
%   58 &     2.74 & flexural in z &   229 &    42.24 & longitudinal \\
%   59 &     2.95 & flexural in y &   236 &    44.60 & torsional    \\
%   60 &     2.95 & flexural in z &   245 &    48.03 & torsional    \\
%   61 &     3.17 & flexural in z &   252 &    50.69 & longitudinal \\
%   62 &     3.17 & flexural in y &   255 &    51.46 & torsional    \\
%   63 &     3.39 & flexural in z &   264 &    54.89 & torsional    \\
%   64 &     3.39 & flexural in y &   271 &    58.32 & torsional    \\
%   65 &     3.43 & torsional     &   274 &    59.14 & longitudinal \\
%   66 &     3.63 & flexural in y &   281 &    61.75 & torsional    \\
%   67 &     3.63 & flexural in z &   288 &    65.18 & torsional    \\
%   68 &     3.87 & flexural in z &  295 &    67.59 & longitudinal \\
%   69 &     3.87 & flexural in y &  298 &    68.62 & torsional    \\
%		\bottomrule
%	\end{tabular}
%	\label{natural_freq_tab}
%\end{table}
%
%
%
%In Figure~\ref{modes_long_x_fig}, the reader can observe the first three 
%longitudinal (traction-compression) modes of vibration of the 
%free-free beam, taking into account or not the mass of the fluid 
%inside the drillstring. The inclusion of the fluid does not change the 
%first three natural frequencies of traction-compression, which are 
%respectively equal to $8.45$, $16.90$ and $25.35~Hz$. This fact 
%had already been evidenced in the thesis of Ritto \cite{ritto2010}.
%However, it is noted that the presence of the fluid causes an inversion 
%in the state of traction-compression, i.e., points before in traction enter 
%into compression and vice versa.
%
%
%\begin{figure}[h]
%	\centering
%	\includegraphics[scale=0.3]{figs/modes/modes_long_x_1.pdf}
%	\includegraphics[scale=0.3]{figs/modes/modes_long_x_2.pdf}
%	\includegraphics[scale=0.3]{figs/modes/modes_long_x_3.pdf}
%	\caption{Illustration of the first three longitudinal (traction-compression) modes of the beam.}
%	\label{modes_long_x_fig}
%\end{figure}
%
%
%Regarding the torsion mechanism, the inclusion of fluid does not affects neither 
%the first three natural frequencies ($3.43$, $6.86$ and $10.29~Hz$) nor the 
%corresponding normal modes, as can be seen in Figure~\ref{modes_tors_x_fig}.
%This is reasonable from the physical point of view, since fill the interior of the beam 
%with a fluid imposes no extra difficulty to twist it, as well as does not facilitates.
%
%\begin{figure}[h]
%	\centering
%	\includegraphics[scale=0.3]{figs/modes/modes_tors_x_1.pdf}
%	\includegraphics[scale=0.3]{figs/modes/modes_tors_x_2.pdf}
%	\includegraphics[scale=0.3]{figs/modes/modes_tors_x_3.pdf}
%	\caption{Illustration of the first three torsional modes of the beam.}
%	\label{modes_tors_x_fig}
%\end{figure}
%
%With respect to the flexural mechanism occurs something different.
%The inclusion of the fluid does not change neither the first ($0.01~Hz$)
%nor the third ($0.05~Hz$) natural frequency, but slightly increases the 
%amplitude of the corresponding modes, Figure~\ref{modes_flex_y_fig}.
%In the case of the second mode, the natural frequency increases from 
%$0.02~Hz$ to $0.03~Hz$, and, as seen in the Figure~\ref{modes_flex_y_fig},
%this is followed by a reflection of the corresponding normal mode.
%It is clear that flexion is the vibration mechanism more sensitive to 
%the inclusion of the fluid.
%
%
%\begin{figure}[h]
%	\centering
%	\includegraphics[scale=0.3]{figs/modes/modes_flex_y_1.pdf}
%	\includegraphics[scale=0.3]{figs/modes/modes_flex_y_2.pdf}
%	\includegraphics[scale=0.3]{figs/modes/modes_flex_y_3.pdf}
%	\caption{Illustration of the first three flexural modes of the beam.}
%	\label{modes_flex_y_fig}
%\end{figure}






